Anatomy-guided Pathology Segmentation

Pathological structures in medical images are typically deviations from the expected anatomy of a patient. While clinicians consider this interplay between anatomy and pathology, recent deep learning algorithms specialize in recognizing either one of the two, rarely considering the patient's body from such a joint perspective. In this paper, we develop a generalist segmentation model that combines anatomical and pathological information, aiming to enhance the segmentation accuracy of pathological features. Our Anatomy-Pathology Exchange (APEx) training utilizes a query-based segmentation transformer which decodes a joint feature space into query-representations for human anatomy and interleaves them via a mixing strategy into the pathology-decoder for anatomy-informed pathology predictions. In doing so, we are able to report the best results across the board on FDG-PET-CT and Chest X-Ray pathology segmentation tasks with a margin of up to 3.3% as compared to strong baseline methods. Code and models will be publicly available at github.com/alexanderjaus/APEx.

==> Latex/Figures/autopet_qual.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth, trim=0 0 360 0,clip]{Latex/Images/autopet.png}
    \includegraphics[width=0.49\linewidth, trim =0 0 0 440, clip]{Latex/Images/Sup_autopet.drawio.pdf}
    \caption{
    (Left:) We show qualitative comparisons against a Mask2Former baseline. The red ground truth is compared against model predictions in green. (Right:) We show two patients in a coronal and sagittal view below. Volumes shown in red, green, and blue denote the lesion ground truth, \methodname\ predictions, and Mask2Former baseline predictions. Best viewed on a screen and in color.}
    \label{fig:enter-label}
\end{figure}

==> Latex/Figures/chest_xray_qual.tex <==
\begin{table*}[h!]
  \centering    
    \begin{tabular}{cccccc}
  \hline
  \textbf{Input} & \textbf{MaskRCNN}  & \textbf{PointRend}  & 
  %\textbf{MaskDINO} & 
  \textbf{M2F} & \textbf{APEx (Ours)} & \textbf{Target}\\
    \midrule
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/gt_18.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/maskrcnn_results_18_annotated.jpg} & \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/pointrend_results_18_annotated.jpg} &
    %\includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/maskdino_results_18_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/mask2former_results_18_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/ours_18_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/gt_18_annotated.jpg} \\

    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/gt_282.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/maskrcnn_results_282_annotated.jpg} & \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/pointrend_results_282_annotated.jpg} &
    %\includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/maskdino_results_282_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/mask2former_results_282_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/ours_282_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/gt_282_annotated.jpg} \\
    \hline
  \end{tabular}
  \caption{Examples of qualitative segmentation results on ChestXDet. Each class is represented by a distinct color. Best viewed on screen with zoom and in color.}
  \label{tab:chestxdet_qualitative_results}
\end{table*}

==> Latex/Figures/chestxdet.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.95}

\begin{table*}[h!]
\caption{ChestXDet
%\cite{liu2020chestxdet10} 
Results.  We highlight the best performance in \textbf{bold} and the second best by \underline{underlining}.}
\label{tab:chestx_result}
\centering
\scriptsize
\begin{tabular}{lccccccc}
\toprule
Pathology & MRCNN
%\cite{he2017mask} 
&Casc. MRCNN
%\cite{cai2018cascade} 
& PointRend
%\cite{kirillov2019pointrend} 
& MaskDino
%\cite{li2023mask} 
& M2F
%\cite{cheng2021mask2former} 
& Ours   \\
\midrule
{Atel}       & $3.92 \pm 1.15 $   &
                      $ 3.97 \pm 0.90 $   &
                      $ \underline{4.22 \pm  1.20}$ &
                      $ 2.77 \pm 0.77$ &
                      $3.83 \pm 0.60$&
                      $\mathbf{4.38 \pm 0.476}$ 
                      \\
{Calc}     & $5.37 \pm 1.72 $   &
                      $ \underline{6.39 \pm 1.89 }$   &
                      $ \mathbf{6.72 \pm  1.75}$ &
                      $ 6.29 \pm 0.86$ &
                      $5.62 \pm 0.91$&
                      $5.80 \pm 1.39$
                      \\
{Card}      & $44.47 \pm 2.51 $  &
                      $ 45.82 \pm 2.15 $   &
                      $ \mathbf{50.03 \pm  1.7}$ &
                      $ 37.18 \pm 1.22$ &
                      $34.24 \pm 5.69$&
                      $\underline{48.00 \pm 1.63}$
                      \\
{Consol}     & $16.87 \pm 0.412 $ &
                      $ 17.65 \pm 1.04 $   &
                      $ 17.74 \pm 0.51$ &
                      $ 18.79 \pm 1.01$ &
                      $\underline{19.06 \pm 1.14}$&
                      $\mathbf{21.32 \pm 0.59}$
                      \\
{D.Nod}      & $10.89 \pm 2.70 $  &
                      $ 13.12 \pm 2.54 $   &
                      $ 12.93 \pm  2.96$ &
                      $ 18.33 \pm 3.15$ &
                      $\underline{18.72 \pm 2.88}$&
                      $\mathbf{25.82 \pm 2.27}$
                      \\
{Eff}          & $8.56 \pm 1.10 $   &
                      $ 8.28 \pm 1.27 $   &
                      $ 8.29  \pm  0.35$ &
                      $ 10.78 \pm 1.09$ &
                      \underline{$12.33 \pm 0.63$}&
                      $\mathbf{11.94 \pm 1.47}$
                      \\
{Emph}         &  $44.47 \pm 2.31 $ &
                      $ 42.89 \pm 2.40 $   &
                      $ 42.46 \pm  3.43$ &
                      $\underline{ 45.9 \pm 4.38}$ &
                      $45.30 \pm 2.04$&
                      $\mathbf{54.94 \pm 2.61}$
                      \\
{Fib}          & $ 10.48 \pm 2.11 $ &
                       $ 10.71 \pm 1.32 $&
                      $ 9.76 \pm  1.69$ &
                      $ 10.31 \pm 2.13$ &
                      $\underline{11.23 \pm 1.85}$&
                      $\mathbf{12.55 \pm 1.39}$ \\
{Fract}          & $7.65 \pm 1.08 $   &
                      $ 6.36 \pm 1.46 $   &
                      $\mathbf{ 10.61 \pm  0.59}$ &
                      $ 8.527 \pm 0.845$ &
                      $7.28 \pm 0.86$&
                      $\underline{9.76 \pm 0.502}$
                      \\
{Mass}              &  $11.59 \pm 2.89 $ &
                      $ 11.93 \pm 3.07 $   &
                      $\mathbf{ 15.66 \pm  1.73}$ &
                      $ \underline{12.39 \pm 1.86}$ &
                      $8.03 \pm 1.40$&
                      $11.94 \pm 1.75$
                      \\
{Nod}             &  $\underline{5.72 \pm 0.53 }$ &
                      $ 5.41 \pm 1.00 $   &
                      $ \mathbf{6.97 \pm  0.79}$ &
                      $ 5.646 \pm 1.47$ &
                      $5.14 \pm 0.59$&
                      $5.48 \pm 0.688$
                      \\
{Pl.Thick} & $4.32 \pm 1.32 $  &
                      $4.43 \pm 0.74 $   &
                      $\mathbf{ 5.12 \pm  1.23}$ &
                      $ 4.28 \pm 0.73$ &
                      $3.70 \pm 0.50$&
                      $\underline{ 4.61 \pm 0.66}$
                      \\
{Pneumo}      &  $4.10 \pm 0.804 $ &
                      $ 3.21 \pm 1.03 $   &
                      $\underline{ 6.40 \pm  0.92}$ &
                      $ 5.64 \pm 1.65$ &
                      $5.84 \pm 1.24$&
                      $\mathbf{6.93 \pm 1.06}$
                      \\
\midrule
mAP & $13.72 \pm 0.41$ & $13.86 \pm 0.70$ & $15.14\pm 0.44$ & $14.38 \pm	0.74$ & $13.87 \pm 0.53$ & $\mathbf{17.20 \pm 0.33}$ \\
\bottomrule
\end{tabular}
\end{table*}

==> Latex/Figures/duke.tex <==
\begin{table}[b]
\caption{Fluid segmentation results on DUKE OCT}
\label{table:duke_results}
\centering
\small
\begin{tabular}{lcccccc}
\toprule
Method & DSC & IoU \\
\midrule
\textbf{DeepLab V3+} & $65.39 \pm 0.69$ & $50.99 \pm 0.69$ \\
\textbf{Mask2Former} & $63.86 \pm 1.26$ & $49.74 \pm 1.26$ \\
\textbf{UNet} & $ 65.29 \pm 1.41 $ & $ 51.70 \pm 1.54$ \\
\midrule
\textbf{Ours (CA)} & $\mathbf{66.13} \pm \mathbf{0.90}$ & $\mathbf{51.97} \pm \mathbf{0.90}$ \\
\bottomrule
\end{tabular}
\end{table}

% Hyperparams img size, augs, batch size, optimizer, lr, max iters
% Unet (512, 512), randomflip, 16, ADAM, 1e-3 w/ reducelronplateau, 90k
% deeplab (512, 512), randomflip, 16, SGD, 1e-2 w/ warmuppolylr, 90k
% m2f (512, 512), randomflip, 16, ADAMW, 1e-4, w/ warmuppolylr, 90k
% apex (512, 512), randomflip, 16, ADAMW, 1e-4 w/ warmuppolylr, 90k


==> Latex/Figures/insights.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\linewidth, trim=0 160 380 0, clip]{Latex/Images/insights.pdf}
    \caption{Qualitative examples, which anatomical structures informed the segmentation for the presented pathology. We show pathologies in red and highlight the most informative anatomies.}
    \label{fig:insights}
\end{figure}

==> Latex/Figures/introfigure.tex <==
\begin{table*}[h!]
  \centering    
    \begin{tabular}{ccccc}
  \hline
  \textbf{Target} & \textbf{\methodname}  & \textbf{M2F~\cite{cheng2021mask2former}}  & 
  \textbf{Target} & \textbf{APEx (Ours)} & \textbf{Target}\\
    \midrule
    \includegraphics[width=0.14\linewidth]{Latex/Images/autopet_qual/Target.png} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/autopet_qual/Apex.png} & \includegraphics[width=0.14\linewidth]{Latex/Images/autopet_qual/M2F_pred.png} &
    %\includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/maskdino_results_18_annotated.jpg} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/autopet_qual/Attended_anatomy_frontal.png} &
    \includegraphics[width=0.14\linewidth]{Latex/Images/autopet_qual/Attended_anatomy_lateral.png} &
    %\includegraphics[width=0.14\linewidth]{Latex/Images/chestxdet/gt_18_annotated.jpg} \\
    \end{tabular}
  \caption{bla bla bla}
  \label{tab:chestxdet_qualitative_results}
\end{table*}

==> Latex/Figures/oct_qual.tex <==
\begin{table*}[t]
  \centering    
    \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c}
  \hline
  \textbf{Input} & \textbf{DeepLabV3+} & \textbf{UNet} & \textbf{M2F} & \textbf{APEx (Ours)} & \textbf{Target}\\
    \midrule
    \includegraphics[width=2cm]{Latex/Images/duke/Raw_image_split_1_image_8.png} & \includegraphics[width=2cm]{Latex/Images/duke/deeplab_split_1_image_8.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/unet_split_1_image_8.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/m2f_split_1_image_8.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/an4path_split_1_image_8.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/groundtruth_split_1_image_8.png} \\

    \includegraphics[width=2cm]{Latex/Images/duke/Raw_image_split_2_image_5.png} & \includegraphics[width=2cm]{Latex/Images/duke/deeplab_split_2_image_5.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/unet_split_2_image_5.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/m2f_split_2_image_5.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/an4path_split_2_image_5.png} &
    \includegraphics[width=2cm]{Latex/Images/duke/groundtruth_split_2_image_5.png} \\
    \hline
  \end{tabular}
  \caption{Qualitative examples of segmentation results on DUKE OCT. Target outline (green), segmentation outline (black) with respective segmentation area (red)}
  \label{tab:duke_qualitative_results}
\end{table*}

==> Latex/Figures/proposed_method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth, 
    height=0.35\linewidth
    ]{cvpr2023-author_kit-v1_1-1/latex/images/Method_final.pdf}
    \caption{Overview of the proposed \methodname\  Method. At each stage, the two decoders exchange information via the communication module.}
    \label{fig:enter-label}
\end{figure*}

==> Latex/Figures/qualitative_examples_autopet.tex <==
\begin{table}
\caption{IoU Validation scores for anatomical knowledge incooperation}
%\vspace{-0.25cm}
\centering
    \begin{tabular}{|cc|}
    \multicolumn{2}{c}{\textbf{Naive Anatomy Incoporation}} \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Baseline}} \\
    Predict P & $ 54.34 \pm 1.46$ \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Pathology Atop Anatomy }} \\
    Predict A+P & $ 56.10 \pm 3.36$ \\
    Predict A+10*P & $ 57.12 \pm 4.17$ \\
    Predict A+142*P & $ 55.89 \pm 3.03$\\
    \hline
    \multicolumn{2}{|c|}{\textbf{Anatomy as Aux Input}}\\
    Predict A+P & $ 56.52 \pm 4.14$ \\
    Predict P & $ 57.23 \pm 2.71$ \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Pretrained Anatomy}}\\
    Predict P & $ 56.64 \pm 3.06$ \\
    \hline
    %\multicolumn{2}{c}%{\textbf{Ours}} \\
    %Shared BB & $ 54.44 \pm 4.14$ \\
    %Shared BB+PD & $ 58.69 \pm 3.63$ \\
    %\methodname &  $\mathbf{59.35} \pm \mathbf{3.18}$ \\
    %\hline
    \end{tabular}\hspace{0.25cm}
    \begin{tabular}{|cc|}

    \multicolumn{2}{c}{\textbf{Architecture Ablations}} \\
    \hline
    %\multicolumn{2}{c}{\textbf{Baseline}} \\
    %Baseline & $ 54.34 \pm 1.46$ \\
    %\hline
    \multicolumn{2}{|c|}{\textbf{Component Sharing}} \\
    Share Backbone (BB) & $ 54.44 \pm 4.14$ \\
    Share BB+Pix Decoder & $ 58.69 \pm 3.63$ \\
    %\vspace{-0.2cm}\\
    \hline
    \multicolumn{2}{|c|}{\textbf{Query Mixing Nonparametric}}\\
    Query Sum & $ 59.56 \pm 3.64$ \\
    Query Sum 2-ways & $ 59.35 \pm 3.18$ \\
    Query Sum skip last & $ 59.68 \pm 2.54$ \\
    Query Mean & $ 59.78 \pm 3.23$ \\
    \hline
    \multicolumn{2}{|c|}{\textbf{Query Mixing Parametric}}\\
    Cross Attention (CA) & $ 59.42 \pm 2.42$ \\
    CA per feature level & $ 58.48 \pm 2.52$ \\
    \hline
    %\multicolumn{2}{c}%{\textbf{Ours}} \\
    %Shared BB & $ 54.44 \pm 4.14$ \\
    %Shared BB+PD & $ 58.69 \pm 3.63$ \\
    %\methodname &  $\mathbf{59.35} \pm \mathbf{3.18}$ \\
    %\hline
    \end{tabular}
    %\caption{On the left we show our Ablations }
    \label{tab:ablations}
    %\vspace{-0.9cm}
\end{table}



==> Latex/Figures/qualitative_examples_autopet_alt.tex <==
\begin{table}[b]
\centering
\caption{Comparison of \methodname\ against multiple SOTA methods. We highlight the \textbf{best} and the \underline{second best} performance. }
\label{tab: autopet results}

% Subheading for the first table
%\textbf{Validation Results}
\small
\begin{tabular}{lcc|ccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{VAL} & & \multicolumn{2}{c}{TEST} \\\cline{2-3}\cline{5-6} \noalign{\vskip 3pt}    
& IoU & BIoU && IoU & BIoU \\
\midrule
Baseline & $55.00 \pm 3.5$ & $54.78 \pm 3.6$  && $53.60 \pm 5.4$ & $53.07 \pm 5.4$  \\
Predict A+P & $54.34 \pm 1.4$ & $54.16 \pm 1.6$  && $55.48 \pm 1.1$ & $55.02 \pm 1.1$  \\
Predict A+10xP & $\underline{57.6 \pm 3.2}$ & $\underline{57.3 \pm 3.3}$  && $\underline{56.4 \pm 1.5}$ & $\underline{55.8 \pm 1.4}$  \\
\midrule
Ours & \textbf{$\mathbf{59.3 \pm 3.1}$} & \textbf{$\mathbf{59.1 \pm 3.1}$}  && \textbf{$\mathbf{57.0 \pm 1.4}$} & \textbf{$\mathbf{56.5 \pm 1.4}$}  \\
\bottomrule
\end{tabular}


% \begin{tabular}{lccccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{Val} & & \multicolumn{2}{c}{Test} \\ & IoU & BIoU && IoU & BIoU \\
% \midrule
% DeepLabV3+\cite{chen2018encoder} & $55.00 \pm 3.55$ & $54.78 \pm 3.68$  && $53.60 \pm 5.45$ & $53.07 \pm 5.43$  \\
% M2F~\cite{cheng2021mask2former} & $54.34 \pm 1.46$ & $54.16 \pm 1.63$  && $55.48 \pm 1.18$ & $55.02 \pm 1.10$  \\
% UNet~\cite{ronneberger2015unet} & $\underline{57.62 \pm 3.24}$ & $\underline{57.38 \pm 3.32}$  && $\underline{56.43 \pm 1.57}$ & $\underline{55.86 \pm 1.49}$  \\
% Ours & \textbf{$\mathbf{59.35 \pm 3.18}$} & \textbf{$\mathbf{59.12 \pm 3.13}$}  && \textbf{$\mathbf{57.05 \pm 1.43}$} & \textbf{$\mathbf{56.57 \pm 1.41}$}  \\
% \bottomrule
% \end{tabular}

% \vspace{2mm} % Add some space between the tables

% % Subheading for the second table
% %\textbf{Test Results}
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Method & IoU TEST & BIoU TEST \\
% \midrule
% DeepLab V3+\cite{chen2018encoder} & \\
% M2F~\cite{cheng2021mask2former} & \\
% UNet~\cite{ronneberger2015unet} & \\
% Ours & \\
% \bottomrule
% \end{tabular}

\end{table}



==> Latex/Figures/qualitative_examples_autopet_old_old.tex <==
\begin{table}
    \begin{tabular}{cc}
    
    \hline
    
    {Prediction Target} & {VAL Dice} \\
    \hline 
    \hline
    
    \multicolumn{2}{c}{\textbf{Baseline}} \\
    P & $ 54.34 \pm 1.46$ \\
    \hline
    \multicolumn{2}{c}{\textbf{Pathology Atop Anatomy }} \\
    A+P  & $ 56.10 \pm 3.36$ \\
    A+10*P & $ 57.12 \pm 4.17$ \\
    A+142*P & $ 55.89 \pm 3.03$\\
    \hline
    \multicolumn{2}{c}{\textbf{Anatomy as Aux Input}}\\
    A+P & $ 56.52 \pm 4.14$ \\
    P & $ 57.23 \pm 2.71$ \\
    \hline
    \multicolumn{2}{c}{\textbf{Pretrained Anatomy}}\\
    P & $ 56.64 \pm 3.06$ \\
    \hline
    %\multicolumn{2}{c}%{\textbf{Ours}} \\
    %Shared BB & $ 54.44 \pm 4.14$ \\
    %Shared BB+PD & $ 58.69 \pm 3.63$ \\
    %\methodname &  $\mathbf{59.35} \pm \mathbf{3.18}$ \\
    %\hline
    \end{tabular}\hspace{0.5cm}
    \begin{tabular}{cc}

    \hline
     
    {Architecture} & {VAL Dice} \\
    \hline 
    \hline
    
    \multicolumn{2}{c}{\textbf{Shared Components}} \\
    Backbone (BB) & $ 54.34 \pm 1.46$ \\
    BB+Pix Decoder  & $ 58.69 \pm 3.62$ \\
    \hline
    \multicolumn{2}{c}{\textbf{Query Mixing}} \\
    Query Sum  & $ 56.10 \pm 3.36$ \\
     & $ 57.12 \pm 4.17$ \\
    A+142*P & $ 55.89 \pm 3.03$\\
    \hline
    \multicolumn{2}{c}{\textbf{Anatomy as Aux Input}}\\
    A+P & $ 56.52 \pm 4.14$ \\
    P & $ 57.23 \pm 2.71$ \\
    \hline
    \multicolumn{2}{c}{\textbf{Pretrained Anatomy}}\\
    P & $ 56.64 \pm 3.06$ \\
    \hline
    %\multicolumn{2}{c}%{\textbf{Ours}} \\
    %Shared BB & $ 54.44 \pm 4.14$ \\
    %Shared BB+PD & $ 58.69 \pm 3.63$ \\
    %\methodname &  $\mathbf{59.35} \pm \mathbf{3.18}$ \\
    %\hline
    \end{tabular}
    
    \caption{On the left we  }
    \label{tab:overview}
\end{table}





\iffalse


\begin{figure*}
    \centering
    \small
    \begin{tabular}{cccc}

\cline{1-2}
Train Setting & IoU VAL 

         &  &

         \multirow{10}{*}{
         \includegraphics[width=0.7\linewidth, height=0.30\linewidth]{Latex/Images/autopet.png}}
    \\
\cline{1-2}
\multicolumn{2}{c}{\textbf{Baseline}} \\
Train Path & $ 54.34 \pm 1.46$ \\
\cline{1-2}
\multicolumn{2}{c}{\textbf{Train Jointly}} \\
Train Joint & $ 56.10 \pm 3.36$ \\
Train Joint 10X & $ 57.12 \pm 4.17$ \\
Joint Joint 142X & $ 55.89 \pm 3.03$\\
\cline{1-2}
\multicolumn{2}{c}{\textbf{Anatomy Input}}\\
Train Joint & $ 56.52 \pm 4.14$ \\
Train Path & $ 57.23 \pm 2.71$ \\
\cline{1-2}
\multicolumn{2}{c}{\textbf{Finetune Anatomy}}\\
Train Path & $ 56.64 \pm 3.06$ \\
\cline{1-2}
\cline{1-2}
\multicolumn{2}{c}{\textbf{Ours}} \\
 % Architecture  & $ IoU VAL \\
\cline{1-2}
Shared BB & $ 54.44 \pm 4.14$ \\
Shared BB+PD & $ 58.69 \pm 3.63$ \\
\methodname &  $\mathbf{59.35} \pm \mathbf{3.18}$ \\
\cline{1-2}
% \caption{Overview of Ablation Experiments}
    \end{tabular} 
    \caption{On the left, we show crossval ablation results on the autoPET. On the right, qualitative comparisons against Mask2Former. }
    \label{fig:autopet_qual}    
\end{figure*}


\fi

\iffalse

\toprule
Train Setting & IoU VAL \\
\midrule
\multicolumn{2}{c}{\textbf{Baseline}} \\
Train Path & $ 54.34 \pm 1.46$ \\
\hline
\multicolumn{2}{c}{\textbf{Train Jointly}} \\
Train Joint & $ 56.10 \pm 3.36$ \\
Train Joint 10X & $ 57.12 \pm 4.17$ \\
Joint Joint 142X & $ 55.89 \pm 3.03$\\
\hline
\multicolumn{2}{c}{\textbf{Anatomy Input}}\\
Train Joint & $ 56.52 \pm 4.14$ \\
Train Path & $ 57.23 \pm 2.71$ \\
\hline
\multicolumn{2}{c}{\textbf{Finetune Anatomy}}\\
Train Path & $ 56.64 \pm 3.06$ \\
\hline
\toprule
\multicolumn{2}{c}{\textbf{Ours}} \\
 % Architecture  & $ IoU VAL \\
\midrule
Shared BB & $ 54.44 \pm 4.14$ \\
Shared BB+PD & $ 58.69 \pm 3.63$ \\
\methodname &  \textbf{$59.35 \pm 3.18$} \\
\bottomrule

\fi
